Learning-driven Physically-aware Large-scale Circuit Gate Sizing

Gate sizing plays an important role in timing optimization after physical design. Existing machine learning-based gate sizing works cannot optimize timing on multiple timing paths simultaneously and neglect the physical constraint on layouts. They cause sub-optimal sizing solutions and low-efficiency issues when compared with commercial gate sizing tools. In this work, we propose a learning-driven physically-aware gate sizing framework to optimize timing performance on large-scale circuits efficiently. In our gradient descent optimization-based work, for obtaining accurate gradients, a multi-modal gate sizing-aware timing model is achieved via learning timing information on multiple timing paths and physical information on multiple-scaled layouts jointly. Then, gradient generation based on the sizing-oriented estimator and adaptive back-propagation are developed to update gate sizes. Our results demonstrate that our work achieves higher timing performance improvements in a faster way compared with the commercial gate sizing tool.

==> doc/abstract.tex <==
\begin{abstract}
Gate sizing plays an important role in timing optimization after physical design.
Existing machine learning-based gate sizing works cannot optimize timing on multiple timing paths simultaneously and neglect the physical constraint on layouts.
They cause sub-optimal sizing solutions and low-efficiency issues when compared with commercial gate sizing tools.
In this work, we propose a learning-driven physically-aware gate sizing framework to optimize timing performance on large-scale circuits efficiently.
In our gradient descent optimization-based work, for obtaining accurate gradients, a multi-modal gate sizing-aware timing model is achieved via learning timing information on multiple timing paths and physical information on multiple-scaled layouts jointly.
Then, gradient generation based on the sizing-oriented estimator and adaptive back-propagation are developed to update gate sizes.
Our results demonstrate that our work achieves higher timing performance improvements in a faster way compared with the commercial gate sizing tool.
\end{abstract}
%Commercial gate sizing tools can achieve them but in a timing-consuming way.
%\textcolor{red}{Commercial gate sizing tools cannot achieve them in a efficient way.}
%Our results indicate that our work achieves 16.29\% WNS improvements and 18.61\% TNS improvements on average compared with the commercial gate sizing tool when optimizing timing performance.
%And it obtains a 6.64$\times$ speedup.
%Gate sizing plays an important role in timing optimization for achieving timing closure after physical design.

==> doc/bk.tex <==
\iffalse
\begin{figure}[!t]
    \centering
    \hspace{-0.2in}
    \subfloat[]{\includegraphics[width=0.5\linewidth]{graph2} \label{fig:graph} }
    \subfloat[]{\centering\includegraphics[width=0.5\linewidth]{image2} \label{fig:image2} }
    \caption{Rich information (a) in optimization flow; (b) on timing paths; (c) on design layouts.  } 
    \label{fig:model}
\end{figure}
\fi

\begin{equation}
    \mathcal{L}^{tot}=\sum_{v \in \mathcal{V}}\{\underbrace{({s}_{v.or}^{tot}-\tau_{v}(\vec{g}_{v.or}))^2 + ({s}_{v.op}^{tot}-\tau_{v}(\vec{g}_{v.op}))^2}_{\text{slack labels}}\} 
\end{equation}


\begin{table*}[t]
    \centering
    \caption{Critical path delay under fresh condition $CPD$-0, critical path delay under 5-year-aged condition $CPD$-5 and logic error rate $ER$ comparisons of approximate circuits generated by our work and others. The units of $CPD$-0 and $CPD$-5 are ps. The unit of $ER$ is \%.}
    \label{tab:2}
    \resizebox{1.0\linewidth}{!}
    %\resizebox{8.8cm}{}}
    { 
\begin{tabular}{c|cccc|cccc|cccc|cccc|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Circuit} & \multicolumn{4}{c}{Initial}            & \multicolumn{4}{c}{ICC2}             & \multicolumn{4}{c}{RL-Sizer}         & \multicolumn{4}{c}{TranSizer}        & \multicolumn{4}{c}{AGD}              & \multicolumn{4}{c}{DAC23}            & \multicolumn{4}{c}{Ours}             \\
                         & $WNS$   & $TNS$      & $NVE$ & $POW.$  & $WNS$   & $TNS$    & $NVE$ & $POW.$  & $WNS$   & $TNS$    & $NVE$ & $POW$   & $WNS$   & $TNS$    & $NVE$ & $POW$   & $WNS$   & $TNS$    & $NVE$ & $POW$   & $WNS$   & $TNS$    & $NVE$ & $POW$   & $WNS$   & $TNS$    & $NVE$ & $POW$   \\ \midrule
dmx\_tx                  & -0.4112 & -2.9417    & 170   & 1.4618  & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1442 & -0.8219  & 75    & 2.7519  & -0.1391 & -0.7998  & 72    & 2.8129  \\
openGFX430               & -0.6688 & -107.1956  & 1042  & 0.9102  & -0.4129 & -30.2528 & 150   & 1.4254  & -0.3976 & -26.2132 & 129   & 1.4789  & -0.4432 & -36.2589 & 192   & 1.3542  & -0.4021 & -36.1854 & 138   & 1.4452  & -0.3814 & -24.0584 & 106   & 1.4899  & -0.3659 & -23.4321 & 98    & 1.4938  \\
ac97\_top                & -0.2281 & -7.7943    & 74    & 1.8342  & -0.0002 & -0.0003  & 2     & 2.3461  & -0.0005 & -0.0012  & 9     & 2.0456  & -0.0004 & -0.0009  & 3     & 2.2548  & -0.0018 & -0.0043  & 9     & 2.2019  & -0.0009 & -0.0021  & 6     & 2.2317  & -0.0001 & -0.0002  & 2     & 2.3502  \\
vga\_enh\_top            & -0.8694 & -237.1859  & 2852  & 4.1925  & -0.0104 & -0.0456  & 14    & 6.4087  & -0.0178 & -0.0829  & 47    & 5.6217  & -0.0154 & -0.0618  & 32    & 5.8214  & -0.0162 & -0.0745  & 42    & 6.0257  & -0.0132 & -0.0579  & 28    & 6.2574  & -0.0093 & -0.0408  & 12    & 6.4589  \\
nova                     & -1.6939 & -1982.8487 & 12007 & 3.6526  & -0.5214 & -28.8674 & 72    & 5.2132  & -0.4621 & -20.2178 & 59    & 5.2831  & -0.5374 & -67.2348 & 348   & 4.9218  & -0.5438 & -35.6218 & 103   & 4.9687  & -0.4879 & -25.6874 & 64    & 5.2749  & -0.4339 & -21.2486 & 31    & 5.3129  \\
mc\_top                  & -0.2500 & -16.7637   & 216   & 1.3899  & -0.0002 & -0.0002  & 1     & 1.6530  & -0.0005 & 0.0013   & 34    & 1.4229  & -0.0003 & -0.0009  & 15    & 1.5478  & -0.0007 & -0.0051  & 68    & 1.4029  & -0.0003 & -0.0007  & 9     & 1.5491  & -0.0002 & -0.0002  & 1     & 1.653   \\
ecg                      & -0.5941 & -771.1540  & 3830  & 13.1050 & -0.0074 & -0.0076  & 3     & 16.6420 & -0.0098 & -0.0158  & 42    & 15.2699 & -0.0081 & -0.0142  & 39    & 15.8438 & -0.0102 & -0.0201  & 65    & 15.0175 & -0.0087 & -0.0132  & 32    & 15.9031 & -0.0062 & -0.0063  & 2     & 15.9078 \\
dmx\_tx                  & -0.4112 & -2.9417    & 170   & 1.4618  & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1442 & -0.8219  & 75    & 2.7519  & -0.1391 & -0.7998  & 72    & 2.8129  \\
usb\_funct               & -0.4830 & -26.1364   & 93    & 1.4151  & -0.1199 & -4.5600  & 48    & 1.5934  & -0.1052 & -4.0214  & 42    & 1.6354  & -0.1256 & -5.2365  & 51    & 1.5567  & -0.1201 & -4.5632  & 49    & 1.5888  & -0.1172 & -4.2561  & 45    & 1.6198  & -0.1002 & -3.514   & 36    & 1.6512  \\
tate\_pairing            & -1.5241 & -2149.5106 & 5272  & 29.2070 & -0.0013 & -0.0055  & 10    & 37.4630 & -0.0021 & -0.0082  & 23    & 33.1258 & -0.0018 & -0.0069  & 15    & 35.6241 & -0.0019 & -0.0072  & 20    & 34.9887 & -0.0016 & -0.0061  & 12    & 36.5897 & -0.0011 & -0.0049  & 8     & 38.0098 \\ \bottomrule
\end{tabular}
        }
\end{table*}

\begin{table}[!t]
	\centering
	\caption{Optimization Runtime (min.) Comparison.} 
	%The critical paths in 18 benchmarks are randomly split into the upper 11 benchmarks for training and the lower 7 for testing.}
	\label{tab:3}
	\resizebox{1.0\linewidth}{!}
	{
		\begin{tabular}{c|c|c|c|c|c|c}
			\toprule
			Circuit & Genetic & V-SASIMI & SimpleRL & ModifyRL & GCNII-RL & Ours   \\ \midrule
			Adder   & 20.51   & 28.49    & \textbf{7.29}     & 13.09    & 12.68    & 8.91   \\
			Bar     & 32.14   & 39.79    & 18.34    & 20.98    & 24.57    & \textbf{17.30}  \\
			Div     & 859.16  & 1182.91  & 312.51   & 502.16   & 232.92   & \textbf{193.86} \\
			Log2    & 681.2   & 702.24   & 209.89   & 189.24   & 165.83   & \textbf{135.05} \\
			Max     & 27.21   & 34.95    & 21.39    & 24.29    & 18.41    & \textbf{15.29}  \\
			Mul     & 213.42  & 224.25   & 78.92    & 149.57   & 61.29    & \textbf{46.72}  \\
			Sin     & 48.20   & 57.61    & 34.19    & 48.91    & 42.13    & \textbf{38.40}  \\
			Sqrt    & 543.23  & 741.98   & 279.82   & 306.86   & 189.71   & \textbf{151.43} \\
			Square  & 38.09   & 44.59    & \textbf{21.59}    & 30.58    & 32.34    & 26.23  \\ \midrule
			Average & 273.68  & 339.65   & 109.33   & 142.85   & 86.65    & \textbf{70.36}  \\ \midrule
		\end{tabular}
	}
\end{table}

\begin{table}[!t]
    \centering
    \caption{Benchmark statistics.} 
    \label{tab:0}
    %\resizebox{0.718\linewidth}{!}
    {
    \begin{tabular}{c|c|c|c|c}
    \toprule
Circuit       & \#gates & \#wires & \#Endps & \#CPs  \\ \cline
dmx\_tx       & 11616   & 11671   & 4671    & 7068   \\
openGFX430    & 11004   & 11156   & 1580    & 18011  \\
ac97\_top     & 4954    & 5046    & 2262    & 3102   \\
vga\_enh\_top & 32727   & 32863   & 17750   & 10860  \\
nova          & 105756  & 107641  & 30427   & 64325  \\ \cline
Total Train   & 166057  & 168377  & 56690   & 103366 \\
mc\_top       & 3943    & 4121    & 1101    & 5660   \\
ecg           & 39992   & 40941   & 7821    & 40963  \\
dmx\_tx       & 11616   & 11671   & 4671    & 3681   \\
usb\_funct    & 6666    & 7000    & 1799    & 6143   \\
tate\_pairing & 153192  & 154720  & 32149   & 73147  \\ \cline
Total Test    & 215409  & 218453  & 47541   & 129594 \\ \bottomrule
\end{tabular}
        }
\end{table}

\begin{table*}[t]
    \centering
    \caption{Critical path delay under fresh condition CPD-0, critical path delay under 5-year-aged condition CPD-5 and logic error rate ER comparisons of approximate circuits generated by our work and others. The units of CPD-0 and CPD-5 are ps. The unit of ER is \%.}
    \label{tab:2}
    \resizebox{1.1\linewidth}{!}
    %\resizebox{8.8cm}{}}
    { 
\begin{tabular}{c|cccc|cccc|cccc|cccc|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Circuit} & \multicolumn{4}{c}{Initial}            & \multicolumn{4}{c}{ICC2}             & \multicolumn{4}{c}{RL-Sizer}         & \multicolumn{4}{c}{TranSizer}        & \multicolumn{4}{c}{AGD}              & \multicolumn{4}{c}{DAC23}            & \multicolumn{4}{c}{Ours}             \\
                         & WNS   & TNS      & NVE & POW  & WNS   & TNS    & NVE & POW  & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   \\ \midrule
dmx                  & -0.4112 & -2.9417    & 170   & 1.4618  & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1442 & -0.8219  & 75    & 2.7519  & -0.1391 & -0.7998  & 72    & 2.8129  \\
GFX430               & -0.6688 & -107.1956  & 1042  & 0.9102  & -0.4129 & -30.2528 & 150   & 1.4254  & -0.3976 & -26.2132 & 129   & 1.4789  & -0.4432 & -36.2589 & 192   & 1.3542  & -0.4021 & -36.1854 & 138   & 1.4452  & -0.3814 & -24.0584 & 106   & 1.4899  & -0.3659 & -23.4321 & 98    & 1.4938  \\
ac97                & -0.2281 & -7.7943    & 74    & 1.8342  & -0.0002 & -0.0003  & 2     & 2.3461  & -0.0005 & -0.0012  & 9     & 2.0456  & -0.0004 & -0.0009  & 3     & 2.2548  & -0.0018 & -0.0043  & 9     & 2.2019  & -0.0009 & -0.0021  & 6     & 2.2317  & -0.0001 & -0.0002  & 2     & 2.3502  \\
vga          & -0.8694 & -237.1859  & 2852  & 4.1925  & -0.0104 & -0.0456  & 14    & 6.4087  & -0.0178 & -0.0829  & 47    & 5.6217  & -0.0154 & -0.0618  & 32    & 5.8214  & -0.0162 & -0.0745  & 42    & 6.0257  & -0.0132 & -0.0579  & 28    & 6.2574  & -0.0093 & -0.0408  & 12    & 6.4589  \\
nova                     & -1.6939 & -1982.8487 & 12007 & 3.6526  & -0.5214 & -28.8674 & 72    & 5.2132  & -0.4621 & -20.2178 & 59    & 5.2831  & -0.5374 & -67.2348 & 348   & 4.9218  & -0.5438 & -35.6218 & 103   & 4.9687  & -0.4879 & -25.6874 & 64    & 5.2749  & -0.4339 & -21.2486 & 31    & 5.3129  \\
mc                & -0.2500 & -16.7637   & 216   & 1.3899  & -0.0002 & -0.0002  & 1     & 1.6530  & -0.0005 & 0.0013   & 34    & 1.4229  & -0.0003 & -0.0009  & 15    & 1.5478  & -0.0007 & -0.0051  & 68    & 1.4029  & -0.0003 & -0.0007  & 9     & 1.5491  & -0.0002 & -0.0002  & 1     & 1.653   \\
ecg                      & -0.5941 & -771.1540  & 3830  & 13.1050 & -0.0074 & -0.0076  & 3     & 16.6420 & -0.0098 & -0.0158  & 42    & 15.2699 & -0.0081 & -0.0142  & 39    & 15.8438 & -0.0102 & -0.0201  & 65    & 15.0175 & -0.0087 & -0.0132  & 32    & 15.9031 & -0.0062 & -0.0063  & 2     & 15.9078 \\
dmx                  & -0.4112 & -2.9417    & 170   & 1.4618  & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1442 & -0.8219  & 75    & 2.7519  & -0.1391 & -0.7998  & 72    & 2.8129  \\
usb               & -0.4830 & -26.1364   & 93    & 1.4151  & -0.1199 & -4.5600  & 48    & 1.5934  & -0.1052 & -4.0214  & 42    & 1.6354  & -0.1256 & -5.2365  & 51    & 1.5567  & -0.1201 & -4.5632  & 49    & 1.5888  & -0.1172 & -4.2561  & 45    & 1.6198  & -0.1002 & -3.514   & 36    & 1.6512  \\
tate          & -1.5241 & -2149.5106 & 5272  & 29.2070 & -0.0013 & -0.0055  & 10    & 37.4630 & -0.0021 & -0.0082  & 23    & 33.1258 & -0.0018 & -0.0069  & 15    & 35.6241 & -0.0019 & -0.0072  & 20    & 34.9887 & -0.0016 & -0.0061  & 12    & 36.5897 & -0.0011 & -0.0049  & 8     & 38.0098 \\ \bottomrule
\end{tabular}
        }
\end{table*}

==> doc/cover.tex <==
{
%\twocolumn[
%\begin{@twocolumnfalse}
%\large

\noindent Dear Editor and Reviewers,

\ \\
Thank you very much for reviewing and editing our submission.
Enclosed is our manuscript entitled \textit{``
	Learning-driven Physically-aware Large-scale Circuit Gate Sizing 
''}.
This is an original paper that has not been published anywhere else.
We look forward to contributing to IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD).
Thank you in advance for your efforts on reviewing and editing.

\ \\
Best regards,

\ \\

\noindent 
Yuyang Ye

%\end{@twocolumnfalse}
%]
}


==> doc/tab-bk.tex <==
\begin{table*}[t]
    \centering
    \caption{Critical path delay under fresh condition CPD-0, critical path delay under 5-year-aged condition CPD-5 and logic error rate ER comparisons of approximate circuits generated by our work and others. The units of CPD-0 and CPD-5 are ps. The unit of ER is \%.}
    \label{tab:2}
    \resizebox{1.0\linewidth}{!}
    %\resizebox{8.8cm}{}}
    { 
\begin{tabular}{c|cccc|cccc|cccc|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Circuit} & \multicolumn{4}{c}{Initial}            & \multicolumn{4}{c}{ICC2}             & \multicolumn{4}{c}{RL-Sizer}         & \multicolumn{4}{c}{TranSizer}        & \multicolumn{4}{c}{AGD}              & \multicolumn{4}{c}{Ours}             \\ \cline{1-25}
                         & WNS   & TNS      & NVE   & POW.  & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   & WNS   & TNS    & NVE & POW   \\
dmx\_tx                  & -0.4112 & -2.9417    & 170   & 1.4618  & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1391 & -0.7998  & 72    & 2.8129  \\ \midrule
openGFX430               & -0.6688 & -107.1956  & 1042  & 0.9102  & -0.4129 & -30.2528 & 150   & 1.4254  & -0.3976 & -26.2132 & 129   & 1.4789  & -0.4432 & -36.2589 & 192   & 1.3542  & -0.4021 & -36.1854 & 138   & 1.4452  & -0.3659 & -23.4321 & 98    & 1.4938  \\
ac97\_top                & -0.2281 & -7.7943    & 74    & 1.8342  & -0.0002 & -0.0003  & 2     & 2.3461  & -0.0005 & -0.0012  & 9     & 2.0456  & -0.0004 & -0.0009  & 3     & 2.2548  & -0.0018 & -0.0043  & 9     & 2.2019  & -0.0001 & -0.0002  & 2     & 2.3502  \\
vga\_enh\_top            & -0.8694 & -237.1859  & 2852  & 4.1925  & -0.0104 & -0.0456  & 14    & 6.4087  & -0.0178 & -0.0829  & 47    & 5.6217  & -0.0154 & -0.0618  & 32    & 5.8214  & -0.0162 & -0.0745  & 42    & 6.0257  & -0.0093 & -0.0408  & 12    & 6.4589  \\
nova                     & -1.6939 & -1982.8487 & 12007 & 3.6526  & -0.5214 & -28.8674 & 72    & 5.2132  & -0.4621 & -20.2178 & 59    & 5.2831  & -0.5374 & -67.2348 & 348   & 4.9218  & -0.5438 & -35.6218 & 103   & 4.9687  & -0.4339 & -21.2486 & 31    & 5.3129  \\
mc\_top                  & -0.2500 & -16.7637   & 216   & 1.3899  & -0.0002 & -0.0002  & 1     & 1.6530  & -0.0005 & 0.0013   & 34    & 1.4229  & -0.0003 & -0.0009  & 15    & 1.5478  & -0.0007 & -0.0051  & 68    & 1.4029  & -0.0002 & -0.0002  & 1     & 1.653   \\
ecg                      & -0.5941 & -771.1540  & 3830  & 13.1050 & -0.0074 & -0.0076  & 3     & 16.6420 & -0.0098 & -0.0158  & 42    & 15.2699 & -0.0081 & -0.0142  & 39    & 15.8438 & -0.0102 & -0.0201  & 65    & 15.0175 & -0.0062 & -0.0063  & 2     & 15.9078 \\
dmx\_tx                  & -0.4112 & -2.9417    & 170   & 1.4618  & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1391 & -0.7998  & 72    & 2.8129  \\
usb\_funct               & -0.4830 & -26.1364   & 93    & 1.4151  & -0.1199 & -4.5600  & 48    & 1.5934  & -0.1052 & -4.0214  & 42    & 1.6354  & -0.1256 & -5.2365  & 51    & 1.5567  & -0.1201 & -4.5632  & 49    & 1.5888  & -0.1002 & -3.514   & 36    & 1.6512  \\
tate\_pairing            & -1.5241 & -2149.5106 & 5272  & 29.2070 & -0.0013 & -0.0055  & 10    & 37.4630 & -0.0021 & -0.0082  & 23    & 33.1258 & -0.0018 & -0.0069  & 15    & 35.6241 & -0.0019 & -0.0072  & 20    & 34.9887 & -0.0011 & -0.0049  & 8     & 38.0098 \\ \bottomrule
\end{tabular}
        }
\end{table*}

\begin{table}[!t]
    \centering
    \caption{Benchmark statistics.} 
    \label{tab:0}
    \resizebox{0.718\linewidth}{!}
    {
    \begin{tabular}{l|l|l|l|l|l|l}
    \toprule
Circuit       & \#gates & \#wires & \#Endps & \#CPs  & NVE & POW\\ \midrule
\textit{DMX}       & 11616   & 11671   & 4671    & 7068  & 170 & 1.4618 \\
\textit{GFX}    & 11004   & 11156   & 1580    & 18011  & 1042 & 0.9102\\
\textit{AC97}     & 4954    & 5046    & 2262    & 3102   \\
\textit{VGA} & 32727   & 32863   & 17750   & 10860  \\
\textit{NOVA}          & 105756  & 107641  & 30427   & 64325  \\ \midrule
Total Train   & 166057  & 168377  & 56690   & 103366 \\ \midrule
\textit{MC}       & 3943    & 4121    & 1101    & 5660   \\ 
\textit{ECQ}           & 39992   & 40941   & 7821    & 40963  \\
\textit{DMX}       & 11616   & 11671   & 4671    & 3681   \\
\textit{USB}    & 6666    & 7000    & 1799    & 6143   \\
\textit{TATE} & 153192  & 154720  & 32149   & 73147  \\ \midrule
Total Test    & 215409  & 218453  & 47541   & 129594 \\ \bottomrule
\end{tabular}
        }
\end{table}

\begin{table*}[t]
    \centering
    \caption{Critical path delay under fresh condition CPD-0, critical path delay under 5-year-aged condition CPD-5 and logic error rate ER comparisons of approximate circuits generated by our work and others. The units of CPD-0 and CPD-5 are ps. The unit of ER is \%.}
    \label{tab:2}
    \resizebox{1.0\linewidth}{!}
    %\resizebox{8.8cm}{}}
    { 
\begin{tabular}{ccccccccccccccccccccc}
\multirow{2}{*}{Circuit} & \multicolumn{4}{c}{ICC2}             & \multicolumn{4}{c}{RL-Sizer}         & \multicolumn{4}{c}{TranSizer}        & \multicolumn{4}{c}{AGD}              & \multicolumn{4}{c}{Ours}             \\
                         & WNS   & TNS    & NVE & POW.  & WNS   & TNS    & NVE & POW.  & WNS   & TNS    & NVE & POW.  & WNS   & TNS    & NVE & POW.  & WNS   & TNS    & NVE & POW.  \\
DMX                      & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1391 & -0.7998  & 72    & 2.8129  \\
GFX                      & -0.4129 & -30.2528 & 150   & 1.4254  & -0.3976 & -26.2132 & 129   & 1.4789  & -0.4432 & -36.2589 & 192   & 1.3542  & -0.4021 & -36.1854 & 138   & 1.4452  & -0.3659 & -23.4321 & 98    & 1.4938  \\
AC97                     & -0.0002 & -0.0003  & 2     & 2.3461  & -0.0005 & -0.0012  & 9     & 2.0456  & -0.0004 & -0.0009  & 3     & 2.2548  & -0.0018 & -0.0043  & 9     & 2.2019  & -0.0001 & -0.0002  & 2     & 2.3502  \\
VGA                      & -0.0104 & -0.0456  & 14    & 6.4087  & -0.0178 & -0.0829  & 47    & 5.6217  & -0.0154 & -0.0618  & 32    & 5.8214  & -0.0162 & -0.0745  & 42    & 6.0257  & -0.0093 & -0.0408  & 12    & 6.4589  \\
NOVA                     & -0.5214 & -28.8674 & 72    & 5.2132  & -0.4621 & -20.2178 & 59    & 5.2831  & -0.5374 & -67.2348 & 348   & 4.9218  & -0.5438 & -35.6218 & 103   & 4.9687  & -0.4339 & -21.2486 & 31    & 5.3129  \\
MC\_TOP                  & -0.0002 & -0.0002  & 1     & 1.6530  & -0.0005 & 0.0013   & 34    & 1.4229  & -0.0003 & -0.0009  & 15    & 1.5478  & -0.0007 & -0.0051  & 68    & 1.4029  & -0.0002 & -0.0002  & 1     & 1.653   \\
ECG                      & -0.0012 & -0.0029  & 7     & 6.7383  & -0.0023 & 0.0079   & 26    & 6.3587  & -0.0017 & 0.0051   & 18    & 6.5128  & -0.0019 & -0.0064  & 20    & 6.4541  & -0.001  & -0.0022  & 5     & 6.7891  \\
ETH                      & -0.1596 & -0.9715  & 92    & 2.4312  & -0.1465 & -0.8521  & 80    & 2.6714  & -0.1632 & -1.2354  & 98    & 2.2144  & -0.1508 & -0.9408  & 89    & 2.5284  & -0.1391 & -0.7998  & 72    & 2.8129  \\
USB                      & -0.1199 & -4.5600  & 48    & 1.5934  & -0.1052 & -4.0214  & 42    & 1.6354  & -0.1256 & -5.2365  & 51    & 1.5567  & -0.1201 & -4.5632  & 49    & 1.5888  & -0.1002 & -3.514   & 36    & 1.6512  \\
TATE                     & -0.0013 & -0.0055  & 10    & 37.4630 & -0.0021 & -0.0082  & 23    & 33.1258 & -0.0018 & -0.0069  & 15    & 35.6241 & -0.0019 & -0.0072  & 20    & 34.9887 & -0.0011 & -0.0049  & 8     & 38.0098
\end{tabular}
        }
\end{table*}


==> doc/tab-revise.tex <==
\begin{table*}[t]
	\centering
    \footnotesize
	\caption{Gate-wise TNS $\tau(\vec{g}_v)$ and gate-wise WNS $\omega(\vec{g}_v)$ prediction accuracy. The unit of ``$MAE$'' is $ps$.}
	\label{tab:model}
	%\resizebox{1.0\linewidth}{!}
{ 
	\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
		\hline
		\multirow{3}{*}{Cir.} & \multicolumn{4}{c|}{DAC22 \cite{guo2022timing}}             & \multicolumn{4}{c|}{DAC23 \cite{wang2023restructure}}         
		& \multicolumn{4}{c|}{Ours Layouts-only}        
		& \multicolumn{4}{c|}{Ours Paths-only}              
		& \multicolumn{4}{c|}{Ours}             \\ \cline{2-21}
		& \multicolumn{2}{c|}{$\tau(\vec{g}_v)$} & \multicolumn{2}{c|}{$\omega(\vec{g}_v)$} & \multicolumn{2}{c|}{$\tau(\vec{g}_v)$} & \multicolumn{2}{c|}{$\omega(\vec{g}_v)$} & \multicolumn{2}{c|}{$\tau(\vec{g}_v)$} & \multicolumn{2}{c|}{$\omega(\vec{g}_v)$} & \multicolumn{2}{c|}{$\tau(\vec{g}_v)$} & \multicolumn{2}{c|}{$\omega(\vec{g}_v)$}	& \multicolumn{2}{c|}{$\tau(\vec{g}_v)$} & \multicolumn{2}{c|}{$\omega(\vec{g}_v)$} \\ \cline{2-21}
		& $R^2$  & $MAE$    & $R^2$  & $MAE$  & $R^2$  & $MAE$    & $R^2$  & $MAE$  & $R^2$  & $MAE$    & $R^2$  & $MAE$  & $R^2$  & $MAE$   & $R^2$  & $MAE$ & $R^2$  & $MAE$    & $R^2$  & $MAE$  \\ \hline \hline
		DMX                     & 0.75 & 44.35  & 0.76    & 36.14  & 0.82 & 38.13  & 0.87    & 27.75  & 0.46 & 88.24  & 0.50    & 72.19  & 0.85 & 14.28  & 0.87    & 11.29  & \textbf{0.96} & \textbf{6.29}  & \textbf{0.95}    & \textbf{3.98}  \\
		GFX                      & 0.71 & 36.21 & 0.74   & 29.34  & 0.76 & 28.15 & 0.81   & 22.98  & 0.51 & 76.52 & 0.53   & 71.93  & 0.82 & 12.54 & 0.86   & 10.89  & \textbf{0.96} & \textbf{5.42} & \textbf{0.98}    & \textbf{3.11}  \\
		AC97                    & 0.78 & 47.56  & 0. 8    & 32.68  & 0.84 & 35.24  & 0.86     & 27.77  & 0.49 & 78.90  & 0.51     & 68.92  & 0.84 & 19.12  & 0.86     & 16.24  & \textbf{0.94} & \textbf{7.88}  & \textbf{0.97}     & \textbf{5.06}  \\
		VGA                      & 0.73 & 56.13  & 0.78   & 42.97  & 0.77 & 45.23  & 0.82    & 36.88  & 0.47 & 94.27  & 0.52    & 82.98  & 0.86 & 17.88  & 0.89    & 14.25  & \textbf{0.94} & \textbf{6.92}  & \textbf{0.97}    & \textbf{3.78}  \\
		NOVA                   & 0.79 & 82.14 & 0.81  & 71.54  & 0.82 & 50.13 & 0.84    & 46.37  & 0.55 & 113.25 & 0.59   & 96.24  & 0.86 & 37.28 & 0.90   & 23.99  & \textbf{0.95} & \textbf{7.99} & \textbf{0.98}    & \textbf{4.28}  \\ \hline
  		Ave.                & 0.75  & 53.28   & 0.78 & 42.54  & 0.81   & 39.38 & 0.84  & 34.43  & 0.50   & 90.23 & 0.53  & 78.45  & 0.84   & 20.22 & 0.88  & 15.33 & \textbf{0.95}  & \textbf{6.50}  & \textbf{0.97}     & \textbf{4.04} \\ \hline \hline
		TOP              & 0.67 & 24.24  & 0.71     & 19.15  & 0.75 & 17.21   & 0.78    & 13.99  & 0.45 & 47.67  & 0.49     & 38.92  & 0.79 & 13.75  & 0.83     & 8.98  & \textbf{0.94} & \textbf{5.23}  & \textbf{0.97}     & \textbf{2.35}   \\
		ECG                      & 0.58 & 37.26   & 0.64    & 27.82  & 0.71 & 29.12   & 0.76    & 27.14  & 0.43 & 72.24   & 0.51   & 67.18  & 0.79 & 14.23  & 0.82    & 12.59  & \textbf{0.90}  & \textbf{4.29}  & \textbf{0.94}     & \textbf{3.20}  \\
		ETH                      & 0.69 & 42.75  & 0.72    & 34.62  & 0.77 & 35.14  & 0.81    & 26.32  & 0.50 & 77.11  & 0.45   & 63.14  & 0.83 & 11.27  & 0.87    & 12.17  & \textbf{0.93} & \textbf{3.97}  & \textbf{0.95}    & \textbf{2.12}  \\
		USB                      & 0.66 & 27.99  & 0.70    & 15.74  & 0.76 & 17.89  & 0.80    & 11.24  & 0.40 & 57.12  & 0.42    & 43.89  & 0.84 & 8.24  & 0.89    & 7.92  & \textbf{0.92} & \textbf{3.12}   & \textbf{0.94}    & \textbf{1.27}  \\
		TATE                     & 0.70 & 98.72  & 0.74    & 89.22 & 0.79 & 57.32  & 0.85    & 49.21 & 0.51 & 131.99  & 0.53   & 118.21 & 0.82 & 20.28  & 0.84    & 16.62 & \textbf{0.94} & \textbf{8.23}  & \textbf{0.96}     & \textbf{6.75} \\ \hline 
		Ave.                & 0.66  & 46.19   & 0.70 & 37.31  & 0.76  & 31.14   & 0.80 & 25.58  & 0.46  & 77.23   & 0.48 & 66.27  & 0.82  & 13.55   & 0.85 & 11.67  & \textbf{0.94}  & \textbf{4.77}  & \textbf{0.95}     & \textbf{3.14} \\ \hline 
	\end{tabular}
}
\end{table*}
